Provable Offline Preference-Based Reinforcement Learning

In this paper, we investigate the problem of offline Preference-based Reinforcement Learning (PbRL) with human feedback where feedback is available in the form of preference between trajectory pairs rather than explicit rewards. Our proposed algorithm consists of two main steps: (1) estimate the implicit reward using Maximum Likelihood Estimation (MLE) with general function approximation from offline data and (2) solve a distributionally robust planning problem over a confidence set around the MLE. We consider the general reward setting where the reward can be defined over the whole trajectory and provide a novel guarantee that allows us to learn any target policy with a polynomial number of samples, as long as the target policy is covered by the offline data. This guarantee is the first of its kind with general function approximation. To measure the coverage of the target policy, we introduce a new single-policy concentrability coefficient, which can be upper bounded by the per-trajectory concentrability coefficient. We also establish lower bounds that highlight the necessity of such concentrability and the difference from standard RL, where state-action-wise rewards are directly observed. We further extend and analyze our algorithm when the feedback is given over action pairs.

==> related.tex <==
\section{Related Works}
\label{sec:related}
In this section we introduce the related works of our paper.

\paragraph{Reinforcement learning from human feedback.}

We recommend readers to refer to the survey \citet{wirth2017survey} for an overview of Preference-based RL (PbRL). PbRL has received considerable attention in the theoretical RL literature \citep{yue2012k,novoseller2020dueling,xu2020preference,pacchiano2021dueling,chen2022human}. However, most of these works consider the online setting and there is only limited attention on designing algorithms specifically tailored to offline RL with rigorous statistical guarantees. To the best of our knowledge, \citet{zhu2023principled} is one of the few works that provide such a guarantee. In addition to the comparison in the introduction, a more detailed comparison between our approach and \citet{zhu2023principled} is discussed in Section~\ref{sec:comparison}. 

\paragraph{Offline RL.}   In offline RL, one of the most critical challenges is addressing the issue of insufficient coverage in the offline data. It is well-known that naive methods are unable to learn the optimal policy in such scenarios \citep{rashidinejad2021bridging}. To tackle this problem, numerous algorithms have been proposed from the theoretical perspectives \citep{liu2020provably, kumar20conservative, jin2021pessimism, rashidinejad2021bridging, uehara2021pessimistic,li2022settling,shi2022pessimistic,jin2020pessimism,xie2021bellman,zhan2022offline}. The most relevant work is \cite{uehara2021pessimistic}, which focuses on offline model-based RL with general function approximation. However, their methods cannot be directly applied to RLHF since per-step rewards are not observable in our setting. Furthermore, even in the standard RL setting, the construction of confidence intervals differs between our approach and theirs. Another related paper is \citet{cheng2022adversarially}, which considers the general offline pessimistic RL framework in the standard setting and also subtract a reference term in their algorithm, similar to ours. However, our motivations of such reference terms are quite different from theirs. A detailed discussion on these differences is deferred to Section~\ref{sec:alg} and Remark~\ref{rem:diff}. 
